TableBank: A Benchmark Dataset for Table Detection and Recognition

We present TableBank, a new image-based table detection and recognition dataset built with novel weak supervision from Word and Latex documents on the internet. Existing research for image-based table detection and recognition usually fine-tunes pre-trained models on out-of-domain data with a few thousand human-labeled examples, which is difficult to generalize on real-world applications. With TableBank that contains 417K high quality labeled tables, we build several strong baselines using state-of-the-art models with deep neural networks. We make TableBank publicly available and hope it will empower more deep learning approaches in the table detection and recognition task. The dataset and models are available at \url{https://github.com/doc-analysis/TableBank}.

==> README <==
KNOWN ISSUES

Even if the compilation is successful, on overleaf the following error message appears during (re)compilation:
===ERROR MESSAGE BEGINNING===
 /usr/local/texlive/2018/texmf-dist/tex/latex/base/ts1enc.dfu, line 115
Missing number, treated as zero.

<to be read again> 
                   F
l.115 ...icodeCharacter{FEFF}{\ifhmode\nobreak\fi}
                                                  
A number should have been here; I inserted `0'.
(If you can't figure out why I needed to see a number,
look up `weird error' in the index to The TeXbook.)
===ERROR MESSAGE END===

